Reliable and Interpretable Drift Detection in Streams of Short Texts

Data drift is the change in model input data that is one of the key factors leading to machine learning models performance degradation over time. Monitoring drift helps detecting these issues and preventing their harmful consequences. Meaningful drift interpretation is a fundamental step towards effective re-training of the model. In this study we propose an end-to-end framework for reliable model-agnostic change-point detection and interpretation in large task-oriented dialog systems, proven effective in multiple customer deployments. We evaluate our approach and demonstrate its benefits with a novel variant of intent classification training dataset, simulating customer requests to a dialog system. We make the data publicly available.

==> chapters/3.1-datasets-generation-back.tex <==
\section{Dataset}

The data used in our study revolves around human utterances, originating in first encounters with textual/verbal customer service centers' representatives. These utterances usually correspond to a closed set of specific intents, while their distribution change as a function of time and trends. As part of the nature of customer service centers, such interactions involve communication between a company and a customer. These interactions often involve personal information and sensitive data, leading companies not to publicly share this information due to agreements, privacy constraints, and laws that protect personally identifiable information (PII). This leads to limited publicly available data on customer service interactions, making it difficult to collect such data and fully understand the nature of these interactions. Due to such constraints, we wish to work with datasets best mimicking fundamental human interactions, for example, \cite{larson-etal-2019-evaluation}; This dataset contains 150 intents, each with 150 samples, resulting in 22,500 samples. This dataset is designed for evaluating the performance of intent classification systems with various day-to-day human interactions, such as asking for general information, applying modifications to existing services, and complaining about unsatisfactory situations, resembling typical customer service interactions. Although aforesaid and other similar intent-detection based datasets resemble typical human interactions, they are usually relatively small in comparison to the vast mass of requests customer service centers face daily, as well as not containing duplicates. In contrast, a large number of duplicated utterances is a typical phenomenon in customer service platforms. In light of such discrepancies between publicly available datasets to fundamental human interactions, we wish to take actions to synthetically modify \cite{larson-etal-2019-evaluation} dataset to match the nature of fundamental human interactions best. First, we wish to enrich the data set with new samples to mimic the customer service centers' vast number of human utterances. To do so, we use \cite{anaby2020not} LAMBADA model, trained on each intent's utterances to create new diverse samples holding the same semantic charge as the original samples. Then, we use \cite{prithivida2021parrot} Parrot model to create up to 5 new paraphrases for each utterance, on top of the original and LAMBADA utterances. Statistics on the new dataset sizes after mentioned techniques can be viewed in \ella{complete}X figure. When observing real disclosed human utterances data originating in multi-domain real call centers, we observe Zipf law over the probability distribution of relative frequency over request length (in tokens), as can be viewed in \ella{complete}X figure. Such a phenomenon is not present in publicly open datasets best resembling human behavior. Due to this, we learn such probability distribution over real call centers data and apply it to the enriched dataset by randomly sampling utterances (with repetitions), for each utterance's token length, to reach some dataset size N (1,000,000 in our case), to fit the learned probability distribution. Such a technique incorporates a large number of duplicated utterances in our dataset, a natural phenomenon in real human utterances. We make the data publicly available.

\begin{figure}[h!]
\centering
\resizebox{1\columnwidth}{!}{
\includegraphics{figures/customer-larson-word-length-dist.jpg}
}
%\vspace{-0.1in}
\caption{Distribution of intent classification examples length from \citet{larson-etal-2019-evaluation} (left), and user requests length in a large-scale customer deployment (right). A bar's height mirrors the relative ratio of utterances with a certain number of words in the dataset.}
\label{fig:request-length}
\end{figure}


\begin{table}[hbt]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrr}
dataset & M & STD & total\\ \hline
original (\citet{larson-etal-2019-evaluation}) & ... & ... & ... \\
\hspace{0.1cm} + generation (\citet{uziel2023}) & ... & ... & ... \\
\hspace{0.1cm} + rephrasing (\citet{prithivida2021parrot})& ... & ... & ... \\
\hspace{0.1cm} + upsampling & ... & ... & ...\\

\end{tabular}
}
\caption{Statistics of the created dataset. Mean (M), standard deviation (STD), and the total amount of requests is reported per each expansion step.}
\label{tbl:dataset-details}
\end{table}


%\ella{explain the nature of the required data and the difficulty to obtain publicly available data (companies cannot publish client data due to agreements, privacy constrains, pii, etc.); the motivation for generation of a semi-synthetic dataset that imitates the nature of user requests towards task-oriented dialog system; approach (rephrasing and generating duplicates), examples and statistics; we make the data publicly available; in terms of order: probably first lambada and then parrot}

%\ella{at the duplicates generation part: we learn a probability distribution of relative frequency over request length (in tokens) from large real-customer data; then, with the synthetic data, for each request length (and probably the final dataset size one needs to decide on), we randomly sample requests (with repetitions) proportionally to their anticipated share in the final dataset}

%\ella{good point re unbalanced distribution of requests that arrive from each individual class -- some classes get most of the traffic, some rarely have anything; when learning stats from cvs, let's also take counts on traffic in each individual class and see if we're willing to imitate this behavior}

%\ella{let's aim at Larson et al. and if time permits at Liu et al. -- both are large and heavily multi-class; I suggest to consider getting rid of the "general questions" (and alike) intent from Liu et al. since it doesn't represent a natural class in any way}

==> chapters/7-appendices.tex <==
\section{Appendix}
\label{sec:appendix}

\subsection{Model-dependent Experiments}
Additional set of experiments was conducted using intent classifier posterior estimates as indicator for data drift. Identical experimental setup was applied, where 95\% of intent training set from CLINC150 (seed data) was used for training SVM classifier with training instances' embeddings. Roughly 5\% of intents were randomly selected and held-out as "novel" at each experiment. The pretrained classifier was then used to classify batches of requests from CLINC150-SUR corresponding to the seed data (before injecting drift), and to the seed data extended with drift requests (starting the drift point). Mean classifier confidence was computed for every request batch yielding a series of observations, which was further inut to the change-point detection module (see Section~\ref{sec:drift-point-detection}).

Drift was detected in less than 20\% of the experiments, compared the 96\% with the model-agnostic approach, highlighting the benefits of the direct access to data for drift detection.

